LLMs4OM: Matching Ontologies with Large Language Models

Ontology Matching (OM), is a critical task in knowledge integration, where aligning heterogeneous ontologies facilitates data interoperability and knowledge sharing. Traditional OM systems often rely on expert knowledge or predictive models, with limited exploration of the potential of Large Language Models (LLMs). We present the LLMs4OM framework, a novel approach to evaluate the effectiveness of LLMs in OM tasks. This framework utilizes two modules for retrieval and matching, respectively, enhanced by zero-shot prompting across three ontology representations: concept, concept-parent, and concept-children. Through comprehensive evaluations using 20 OM datasets from various domains, we demonstrate that LLMs, under the LLMs4OM framework, can match and even surpass the performance of traditional OM systems, particularly in complex matching scenarios. Our results highlight the potential of LLMs to significantly contribute to the field of OM.

==> docs/method.tex <==
% As shown in \ref{llms4ontomap}, our framework consists of four main components: (1) parser and concept representations, (2) a retriever that returns top-K candidate from $KB(O_{target})$ for a given query $Q(O_{source})$, (3) an LLM that generates a response for each top-K candidates to whatever they match with source concept or not, and (4) post-processing that do the final filtering based on LLM and retrieval confidence scores. 

% Following a quick preprocessing stage (lowercase texts and punctuation removals), 
